AdaWeather: Adaptively Mixing Probabilistic Weather Forecasts with Logarithmic Regret

Recent advances in machine learning have produced probabilistic weather forecasting models comparable to state-of-the-art numerical weather predictors. But no model consistently dominates spatio-temporally, and relative performance is highly context-dependent. This motivates adaptive methods for combining multiple forecasts to obtain improvements and robustness. While combined forecasts have been proposed in the literature, these are achieved either through supervised learning or through prediction with expert advice methods. We introduce AdaWeather, an adaptive framework that combines many probabilistic forecasts using both machine learning as well as mixture of experts to arrive at a unified improved probabilistic forecast. While traditional expert methods develop the regret bounds with respect to the best single expert in hindsight, we extend the algorithm and analysis to show our method has logarithmic regret compared to the best static mixture of experts in hindsight. Empirically, we focus on forecasting temperature, and observe improvements over existing methods.

==> architecture.tex <==
% architecture.tex
% Pipeline figure for AdaWeather. Standalone TikZ; no external assets.
% Required packages (already loaded by main.tex):
%   tikz, tikzlibrary positioning, arrows.meta, fit, calc, backgrounds,
%   shapes.geometric, shapes.misc, shadows.

% Wong colorblind-safe palette (matches paper_style.py used by other plots).
% Offline branch = blue (#0072B2), Online = vermillion (#D55E00),
% Output = green (#009E73), Truth/feedback = black with red accent.

\definecolor{wongBlue}{HTML}{0072B2}
\definecolor{wongVerm}{HTML}{D55E00}
\definecolor{wongGreen}{HTML}{009E73}
\definecolor{wongPurp}{HTML}{CC79A7}
\definecolor{wongSky}{HTML}{56B4E9}
\definecolor{wongOrng}{HTML}{E69F00}
\definecolor{wongYell}{HTML}{F0E442}
\definecolor{phaseBlueBg}{HTML}{E8F2F9}
\definecolor{phaseVermBg}{HTML}{FAEBE3}

\begin{figure}[t]
\centering
\resizebox{0.95\linewidth}{!}{%
\begin{tikzpicture}[
  >={Stealth[length=2.6mm,width=2.2mm]},
  font=\small\sffamily,
  node distance=4mm and 6mm,
  expert/.style={draw=wongBlue!70!black, line width=0.5pt,
                 rounded corners=1.5pt, fill=white,
                 minimum width=18mm, minimum height=6.5mm, align=center,
                 inner sep=2pt, font=\footnotesize\sffamily},
  unetblock/.style={draw=wongBlue!75!black, line width=0.7pt,
                    rounded corners=2.5pt, fill=wongBlue!12,
                    align=center, inner sep=4pt, font=\small\sffamily,
                    minimum height=12mm},
  pseudoblock/.style={draw=wongBlue!75!black, line width=0.7pt,
                      rounded corners=2.5pt, fill=wongBlue!22,
                      align=center, inner sep=4pt, font=\small\sffamily,
                      minimum height=11mm},
  vtblock/.style={draw=wongVerm!80!black, line width=0.7pt,
                  rounded corners=2.5pt, fill=wongVerm!15,
                  align=center, inner sep=4pt, font=\small\sffamily,
                  minimum height=14mm},
  outblock/.style={draw=wongGreen!75!black, line width=0.7pt,
                   rounded corners=2.5pt, fill=wongGreen!18,
                   align=center, inner sep=4pt, font=\small\sffamily,
                   minimum height=12mm},
  truthblock/.style={draw=black!80, line width=0.5pt,
                     rounded corners=2pt, fill=gray!8,
                     align=center, inner sep=3pt, font=\footnotesize\sffamily},
  arrow/.style={line width=0.6pt, ->, color=black!75},
  thickarrow/.style={line width=0.9pt, ->, color=black!85},
  feedback/.style={line width=0.7pt, ->, dashed,
                   color=wongVerm!90!black, dash pattern=on 2.5pt off 1.5pt},
  glabel/.style={font=\scriptsize\itshape\sffamily, color=black!55},
  phaselabel/.style={font=\small\bfseries\sffamily, anchor=south west},
  edgelabel/.style={font=\scriptsize\sffamily, fill=white,
                    inner sep=0.6pt, color=black!70},
]

% =====================================================================
% LEFT: experts column
% =====================================================================
\node[expert] (e1) {FCN3};
\node[expert, below=2.5mm of e1] (e2) {FGN};
\node[expert, below=2.5mm of e2] (e3) {GenCast};
\node[expert, below=2.5mm of e3] (e4) {IFS-ENS};
\node[expert, below=2.5mm of e4] (e5) {GEM};

% Bracket and group label
\node[glabel, above=1.5mm of e1, anchor=south,
      font=\footnotesize\sffamily\itshape] (eGroupLabel)
      {$N{=}5$ probabilistic experts};
\node[glabel, below=0.6mm of eGroupLabel, anchor=north]
      {(predictive CDFs $F_{n,t}$)};

\coordinate (etop) at ($(e1.north east)+(2.5mm, 1.5mm)$);
\coordinate (ebot) at ($(e5.south east)+(2.5mm, -1.5mm)$);
\draw[gray!55, line width=0.5pt]
  (etop) -- ($(etop)+(1.5mm,0)$) -- ($(ebot)+(1.5mm,0)$) -- (ebot);

% =====================================================================
% TOP ROW: OFFLINE branch
% =====================================================================
\node[unetblock, right=22mm of e1.east, anchor=west, yshift=-2mm,
      minimum width=42mm] (unet)
      {U-Net spatial aggregator
       \\[1pt]
       {\scriptsize encoder--decoder, FiLM lead-time}
       \\[1pt]
       {\scriptsize per-pixel softmax weights $w \in \R^{N{\times}H{\times}W}$}};

\node[pseudoblock, right=8mm of unet, minimum width=34mm] (pseudo)
      {U-Net pseudo-expert
       \\[1pt]
       {\scriptsize $F_{N{+}1,t} = \sum_{n} w_n\,F_{n,t}$}};

% =====================================================================
% BOTTOM ROW: ONLINE branch + output
% =====================================================================
\node[vtblock, below=20mm of pseudo, minimum width=40mm] (vt)
      {VT-MOE online aggregator
       \\[1pt]
       {\scriptsize measure $\mu_t$ on simplex $\Theta \subset \R^{N{+}1}$}
       \\[1pt]
       {\scriptsize closed-form CDF (Eq.~\ref{eq:Ft_explicit})}};

\node[outblock, right=10mm of vt, minimum width=24mm] (out)
      {Forecast CDF
       \\[1pt]
       $\hat F_t(y)$};

\node[truthblock, below=5.5mm of out] (truth)
      {ERA5 truth $y_t$};

% =====================================================================
% ARROWS — experts → U-Net and bypassing to VT-MOE
% =====================================================================
% Arrow stub from each expert to a vertical bus
\foreach \i in {1,2,3,4,5}{%
  \draw[arrow] (e\i.east) -- ($(e\i.east)+(7mm,0)$);
}
% Vertical bus at x = e.east + 7mm; pull bus locations from e1/e5
\coordinate (busTop) at ($(e1.east)+(7mm,0)$);
\coordinate (busBot) at ($(e5.east)+(7mm,0)$);
\coordinate (busMid) at ($(e3.east)+(7mm,0)$);
\draw[line width=0.7pt, color=black!70] (busTop) -- (busBot);

% Bus → U-Net (top route, with mid-arrow label)
\coordinate (toUnet) at ($(unet.west)+(0,-2mm)$);
\draw[arrow] (busMid) -| (toUnet)
      node[edgelabel, pos=0.25, above=0.5mm]{$\{F_{n,t}\}_{n=1}^N$};

% Bus → VT-MOE (bottom route, bypass under the U-Net branch)
\coordinate (vtTopLeft) at ($(vt.west)+(0,3mm)$);
\draw[arrow, color=black!60] (busBot) |- (vtTopLeft);

% U-Net → pseudo-expert
\draw[thickarrow] (unet.east) -- (pseudo.west)
      node[edgelabel, midway, above=0.5mm]{weights $w$};

% Pseudo-expert → VT-MOE (joins as the (N+1)-th expert)
\draw[thickarrow] (pseudo.south) -- ($(pseudo.south)+(0,-4mm)$)
                  -| node[edgelabel, near start, right=0.8mm]
                       {$F_{N{+}1,t}$}
                  ([xshift=-3mm]vt.north);

% VT-MOE → output
\draw[thickarrow] (vt.east) -- (out.west);

% Output → truth (compute CRPS)
\draw[arrow] (out.south) -- ($(out.south)+(0,-3mm)$)
                          -| ([yshift=2mm]truth.north);

% Truth → VT-MOE (feedback): observe y_t, update weights via CRPS
\draw[feedback] (truth.west) -| node[edgelabel, near start, above=0.6mm,
                                      color=wongVerm!85!black,
                                      font=\scriptsize\sffamily\bfseries]
                                     {CRPS update}
                ([xshift=4mm]vt.south);

% =====================================================================
% PHASE LABELS (above the two branches)
% =====================================================================
\node[phaselabel, color=wongBlue!75!black,
      above=2mm of unet.north west, anchor=south west]
      {OFFLINE  \scriptsize\itshape\textcolor{black!55}{train on 2019--2022 ERA5}};

\node[phaselabel, color=wongVerm!75!black,
      below=2mm of vt.south west, anchor=north west]
      {ONLINE  \scriptsize\itshape\textcolor{black!55}{adapt at test time}};

% Subtle background bands to group offline / online phases
\begin{pgfonlayer}{background}
  \node[fit=(unet)(pseudo), inner sep=4mm,
        rounded corners=3pt, fill=phaseBlueBg, draw=none,
        line width=0pt] {};
  \node[fit=(vt)(out), inner sep=4mm,
        rounded corners=3pt, fill=phaseVermBg, draw=none,
        line width=0pt] {};
\end{pgfonlayer}

\end{tikzpicture}%
}
\caption{\textbf{AdaWeather pipeline.} Five probabilistic weather
experts $\{F_{n,t}\}_{n=1}^N$ feed both an offline U-Net spatial
aggregator (top, blue) and the online VT-MOE aggregator (bottom,
vermillion). The U-Net produces per-pixel convex weights $w$ and is
treated, at inference time, as the
$(N{+}1)$\textsuperscript{th} pseudo-expert $F_{N{+}1,t}$. VT-MOE
maintains a measure $\mu_t$ over the $(N{+}1)$-simplex and emits the
final predictive CDF $\hat F_t$ in closed form
(Eq.~\ref{eq:Ft_explicit}). The dashed feedback arrow shows the
CRPS-driven update of $\mu_t$ once the ERA5 truth $y_t$ is observed.
The hybrid inherits the offline branch's exploitation of historical
error structure and the online branch's logarithmic regret guarantee
against the best static convex \emph{mixture} of experts in hindsight
(Theorem~\ref{thm:reg}).}
\label{fig:architecture}
\end{figure}

